VideoMatch: Matching based Video Object Segmentation

Video object segmentation is challenging yet important in a wide variety of applications for video analysis. Recent works formulate video object segmentation as a prediction task using deep nets to achieve appealing state-of-the-art performance. Due to the formulation as a prediction task, most of these methods require fine-tuning during test time, such that the deep nets memorize the appearance of the objects of interest in the given video. However, fine-tuning is time-consuming and computationally expensive, hence the algorithms are far from real time. To address this issue, we develop a novel matching based algorithm for video object segmentation. In contrast to memorization based classification techniques, the proposed approach learns to match extracted features to a provided template without memorizing the appearance of the objects. We validate the effectiveness and the robustness of the proposed method on the challenging DAVIS-16, DAVIS-17, Youtube-Objects and JumpCut datasets. Extensive results show that our method achieves comparable performance without fine-tuning and is much more favorable in terms of computational time.

==> fig_failure.tex <==
% !TEX root = 1636.tex
\setlength{\figwidth}{0.25\textwidth}

\begin{figure}[t]
	%\vspace{0.1cm}
	\begin{center}
		\begin{subfigure}[b]{0.98\figwidth}% 
			\includegraphics[width=\linewidth]{Figs/fail/f4.png} \\
		\end{subfigure}
		\begin{subfigure}[b]{0.98\figwidth}% 
			\includegraphics[width=\linewidth]{Figs/fail/f4_2.png} \\
		\end{subfigure}\hfill
		\begin{subfigure}[b]{0.98\figwidth}% 
			\includegraphics[width=\linewidth]{Figs/fail/f5.png} \\
		\end{subfigure}
		\begin{subfigure}[b]{0.98\figwidth}% 
			\includegraphics[width=\linewidth]{Figs/fail/f5_2.png} \\
		\end{subfigure}
	\end{center}
	%\vspace{-1cm}
	\caption{\tb{Failure cases of our approach.} For each case, we show the results of our approach at the beginning and toward the end of the video sequence.}
	\label{fig:failure}
	%\vspace*{-0.3cm}
\end{figure}

